Utility-driven Optimization of TTL Cache Hierarchies under Network Delays

We optimize hierarchies of Time-to-Live (TTL) caches under random network delays. A TTL cache assigns individual eviction timers to cached objects that are usually refreshed upon a hit where upon a miss the object requires a random time to be fetched from a parent cache. Due to their object decoupling property, TTL caches are of particular interest since the optimization of a per-object utility enables service differentiation. However, state-of-the-art exact TTL cache optimization does not extend beyond single TTL caches, especially under network delays. In this paper, we leverage the object decoupling effect to formulate the non-linear utility maximization problem for TTL cache hierarchies in terms of the exact object hit probability under random network delays. We iteratively solve the utility maximization problem to find the optimal per-object TTLs. Further, we show that the exact model suffers from tractability issues for large hierarchies and propose a machine learning approach to estimate the optimal TTL values for large systems. Finally, we provide numerical and data center trace-based evaluations for both methods showing the significant offloading improvement due to TTL optimization considering the network delays.

==> Evaluations/Acc_delay_4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2in,
height=0.8in,
scale only axis,
xmin=1,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={Number of caches},
ylabel style={font=\color{white!15!black}},
ylabel={Aggregate \\ Utility},
 ylabel style={align=center},
 xlabel style={yshift=0.2cm},
axis background/.style={fill=white},
title style={font=\bfseries},
axis x line*=bottom,
axis y line*=left,
 xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=south west,
]
\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);
\addplot [color=mycolor1, mark=asterisk, only marks, mark options={thick,solid, mycolor1}]
  table[row sep=crcr]{%
1	-4.4005543\\
2	-2.7004775\\
3	-5.68311231\\
4	-8.38186406\\
};
\addlegendentry{$\text{TTL}_{\text{analy.}}$}



\addplot [color=mycolor2, mark=o, only marks, mark options={solid, thick, mycolor2}]
  table[row sep=crcr]{%
1    -4.695786807780189 \\
2 -2.903157031971657\\
3 -5.984159586966149\\
4 -9.112116411516553\\
5 -12.315873205670204\\
6 -15.56450945315369\\
7 -18.762743923444\\
8 -21.909980081430355\\
9 -24.92137247249392\\
10 -28.222738836428867\\
11 -31.304627910845927\\
12 -34.45495696808411\\
13 -37.66726622098249\\
14 -40.7673622643365\\
15 -43.82804723427496\\
16 -47.14111821270257\\
17 -50.298417793643054\\
18 -53.1118002508367\\
19 -56.511213269353355\\
20 -59.72510309201196\\
21 -62.954568155323706\\
};
\addlegendentry{TTL\textsubscript{GNN}}

% \addplot [color=mycolor2, only marks, mark=o, mark options={solid, mycolor2}]
%   table[row sep=crcr]{%
% 1	-4.00787331328347\\
% 2	-3.03483953241433\\
% 3	-5.71785317849144\\
% 4	-8.47863884051534\\
% };
% \addlegendentry{LRU}

\end{axis}

\end{tikzpicture}%

==> Figs/MAP_single_new.tex <==
\ifx\XFigwidth\undefined\dimen1=0pt\else\dimen1\XFigwidth\fi
\divide\dimen1 by 5588
\ifx\XFigheight\undefined\dimen3=0pt\else\dimen3\XFigheight\fi
\divide\dimen3 by 4024
\ifdim\dimen1=0pt\ifdim\dimen3=0pt\dimen1=4143sp\dimen3\dimen1
  \else\dimen1\dimen3\fi\else\ifdim\dimen3=0pt\dimen3\dimen1\fi\fi
\tikzpicture[x=+\dimen1, y=+\dimen3]
{\ifx\XFigu\undefined\catcode`\@11
\def\temp{\alloc@1\dimen\dimendef\insc@unt}\temp\XFigu\catcode`\@12\fi}
\XFigu4143sp
% Uncomment to scale line thicknesses with the same
% factor as width of the drawing.
%\pgfextractx\XFigu{\pgfqpointxy{1}{1}}
\ifdim\XFigu<0pt\XFigu-\XFigu\fi
\pgfdeclarearrow{
  name = xfiga0,
  parameters = {
    \the\pgfarrowlinewidth \the\pgfarrowlength \the\pgfarrowwidth},
  defaults = {
	  line width=+7.5\XFigu, length=+120\XFigu, width=+60\XFigu},
  setup code = {
    % miter protrusion = thk * sqrt(wd^2 + (tipmv*len)^2) / (2 * wd)
    \dimen7 2.15\pgfarrowlength\pgfmathveclen{\the\dimen7}{\the\pgfarrowwidth}
    \dimen7 2\pgfarrowwidth\pgfmathdivide{\pgfmathresult}{\the\dimen7}
    \dimen7 \pgfmathresult\pgfarrowlinewidth
    \pgfarrowssettipend{+\dimen7}
    \pgfarrowssetbackend{+-\pgfarrowlength}
    \dimen9 -0.5\pgfarrowlinewidth
    \pgfarrowssetvisualbackend{+\dimen9}
    \pgfarrowssetlineend{+-0.5\pgfarrowlinewidth}
    \pgfarrowshullpoint{+\dimen7}{+0pt}
    \pgfarrowsupperhullpoint{+-\pgfarrowlength}{+0.5\pgfarrowwidth}
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {\pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{-\pgfarrowlength}{0.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{-\pgfarrowlength}{-0.5\pgfarrowwidth}}
    \pgfusepathqstroke
  }
}
%\draw (4000,-2575) [rounded corners=+105\XFigu] rectangle (2650,-1890);
%\clip(2283,-5359) rectangle (8871,-1335);
\tikzset{inner sep=+0pt, outer sep=+0pt}
\pgfsetlinewidth{+7.5\XFigu}
\draw[thick]  (5062,-2327) circle [radius=+506];
\draw[thick]  (5062,-4846) circle [radius=+506];
\draw[thick]  (735	7,-3510) circle [radius=+506];
\pgfsetarrows{[line width=15\XFigu, width=75\XFigu]}

\pgfsetarrowsstart{xfiga0}


\draw (7695,-3150) arc[start angle=+137.5, end angle=+-129.8, radius=+467.5];
\draw [thick](5085,-2825)--(5085,-4340);
\draw [thick](6975,-3206)--(5520,-2531);
\pgfsetarrows{-xfiga0}
\draw[thick] (6975,-3825)--(5520,-4655);
%\draw[thick] (2815,-3330) rectangle (3875,-4140);
\pgfsetarrowsend{xfiga0}
%\draw (3350,-5040)--(3350,-4140);
%\draw (3350,-3330)--(3350,-2570);
%\pgftext[base,left,at=\pgfqpointxy{2990}{-3825}] {\fontsize{20}{14.4}\textbf{Cache}}
\pgftext[base,left,at=\pgfqpointxy{5010}{-2407}] {\fontsize{17}{30}$0$}
\pgftext[base,left,at=\pgfqpointxy{5010}{-4895}] {\fontsize{17}{30}$1$}
\pgftext[base,left,at=\pgfqpointxy{7280}{-3600}] {\fontsize{17}{30}$F$}
\pgftext[base,left,at=\pgfqpointxy{4560}{-3735}] {\fontsize{15}{14.4}$\lambda_T,0$}
\pgftext[base,left,at=\pgfqpointxy{6300}{-4450}] {\fontsize{15}{14.4}$\lambda_\Delta,0$}
\pgftext[base,left,at=\pgfqpointxy{6210}{-2755}] {\fontsize{15}{14.4}$0,\lambda$}
%\pgftext[base,left,at=\pgfqpointxy{2915}{-3070}] {\fontsize{20}{14.4}\textbf{Cache}}
%\pgftext[base,left,at=\pgfqpointxy{5755}{-1685}] {\fontsize{20}{14.4}\textbf{MAP}}
%\pgftext[base,left,at=\pgfqpointxy{3000}{-2280}] {\fontsize{17}{14.4}\textbf{Server}}
\pgftext[base,left,at=\pgfqpointxy{8060}{-3530}] {\fontsize{15}{14.4}$0,\lambda$} 
%\pgftext[base,left,at=\pgfqpointxy{3280}{-5230}] {\fontsize{15}{14.4}$\lambda$} 

\endtikzpicture%


==> Figs/Tree.tex <==
\ifx\XFigwidth\undefined\dimen1=0pt\else\dimen1\XFigwidth\fi
\divide\dimen1 by 3534
\ifx\XFigheight\undefined\dimen3=0pt\else\dimen3\XFigheight\fi
\divide\dimen3 by 2907
\ifdim\dimen1=0pt\ifdim\dimen3=0pt\dimen1=4143sp\dimen3\dimen1
  \else\dimen1\dimen3\fi\else\ifdim\dimen3=0pt\dimen3\dimen1\fi\fi
\tikzpicture[x=+\dimen1, y=+\dimen3]
{\ifx\XFigu\undefined\catcode`\@11
\def\temp{\alloc@1\dimen\dimendef\insc@unt}\temp\XFigu\catcode`\@12\fi}
\XFigu4143sp
% Uncomment to scale line thicknesses with the same
% factor as width of the drawing.
%\pgfextractx\XFigu{\pgfqpointxy{1}{1}}
\ifdim\XFigu<0pt\XFigu-\XFigu\fi
%\clip(2733,-4875) rectangle (6267,-1968);
\tikzset{inner sep=+0pt, outer sep=+0pt}
\pgfsetlinewidth{+7.5\XFigu}
\draw (2845,-3825)  rectangle(3945,-4725);
\draw (5130,-3825) rectangle (6230,-4725);
\draw (3915,-1980) rectangle(5015,-2880);
\draw (3385,-3825)--(4455,-2880);
\draw (4455,-2880)--(5670,-3825);
\pgftext[base,left,at=\pgfqpointxy{4280}{-2500}] {\fontsize{22}{16.4}$C_3$}
\pgftext[base,left,at=\pgfqpointxy{3190}{-4380}] {\fontsize{22}{16.4}$C_1$}
\pgftext[base,left,at=\pgfqpointxy{5490}{-4380}] {\fontsize{22}{16.4}$C_2$}

\endtikzpicture%


==> Figs/Utility_log_comparison_algs_line_cache_MMM.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2in,
height=1.8in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=4,
xlabel style={font=\color{white!15!black}},
xlabel={delay ratio},
ymin=-1,
ymax=-0.65,
ylabel style={font=\color{white!15!black}},
ylabel={objective fun},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Log10 utility 2 node line capacity 4 MMM},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black, line width= 0.001\linewidth},legend pos=outer north east]

\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);

\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
1e-05	-0.70123213113284\\
0.5	-0.701227663926867\\
1	-0.701235648979453\\
1.5	-0.701234880411657\\
2	-0.701234318361529\\
2.5	-0.701233864566979\\
3	-0.701233520544472\\
3.5	-0.701233244983363\\
4	-0.701233021077053\\
};
\addlegendentry{TTL ideal}

\addplot [color=mycolor2, mark=asterisk, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
1e-05	-0.701232\\
0.5	-0.732855\\
1	-0.765298\\
1.5	-0.796218\\
2	-0.825137\\
2.5	-0.852082\\
3	-0.877215\\
3.5	-0.900727\\
4	-0.922795\\
};
\addlegendentry{TTL ideal @ 0}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
1e-05	-0.777595981218839\\
0.5	-0.779581091041224\\
1	-0.773612299203485\\
1.5	-0.775463875962976\\
2	-0.781689194733771\\
2.5	-0.780181632070585\\
3	-0.780348582548516\\
3.5	-0.777561439000427\\
4	-0.77768983311286\\
};
\addlegendentry{TTL minTTL sim}

\addplot [color=mycolor4, mark=asterisk, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
1e-05	-0.87005936711723\\
0.5	-0.876290959370905\\
1	-0.88461250429854\\
1.5	-0.890629313301067\\
2	-0.892588278369335\\
2.5	-0.896752574565733\\
3	-0.903503023771576\\
3.5	-0.90930549659012\\
4	-0.905751006366452\\
};
\addlegendentry{TTL LRU sim}

\addplot [color=mycolor5, mark=asterisk, mark options={solid, mycolor5}]
  table[row sep=crcr]{%
0	-0.97975631814955\\
0.1	-0.922904195885581\\
0.2	-0.885580912965942\\
0.3	-0.859813030548583\\
0.4	-0.844837429221266\\
0.5	-0.830756968766493\\
0.6	-0.822087518719318\\
0.7	-0.813117443759141\\
0.8	-0.811599847696792\\
0.9	-0.807123490384572\\
1	-0.801546891887605\\
1.1	-0.799324614021616\\
1.2	-0.799326890738749\\
1.3	-0.794933016822293\\
1.4	-0.795181330027942\\
1.5	-0.798613748016088\\
1.6	-0.797064147291831\\
1.7	-0.797189853637946\\
1.8	-0.793300801114721\\
1.9	-0.792708986675381\\
2	-0.792901998386384\\
2.1	-0.794881611196387\\
2.2	-0.791726707090331\\
2.3	-0.793375342759932\\
2.4	-0.79420255131937\\
2.5	-0.797547868965914\\
2.6	-0.798545583899439\\
2.7	-0.795254850022788\\
2.8	-0.796593366404698\\
2.9	-0.801083609698383\\
3	-0.798218528759677\\
3.1	-0.798250824561339\\
3.2	-0.799372024714118\\
3.3	-0.800455553605268\\
3.4	-0.801250500944081\\
3.5	-0.800217201664523\\
3.6	-0.800920340279848\\
3.7	-0.801533811492209\\
3.8	-0.802475571816072\\
3.9	-0.800414190390169\\
4	-0.804045834472467\\
};
\addlegendentry{LRU}

\addplot [color=mycolor6, mark=o, mark options={solid, mycolor6}]
  table[row sep=crcr]{%
1e-05	-0.700506135473052\\
0.5	-0.702780089235904\\
1	-0.700233881700606\\
1.5	-0.70132558970691\\
2	-0.701865628503026\\
2.5	-0.704973449899888\\
3	-0.703435719375941\\
3.5	-0.703863708551098\\
4	-0.699908141411171\\
};
\addlegendentry{TTL extend timers}

\addplot [color=mycolor7, mark=square, mark options={solid, mycolor7}]
  table[row sep=crcr]{%
1e-05	-0.702337615796576\\
0.5	-0.699958760952574\\
1	-0.699777785502701\\
1.5	-0.702027124374383\\
2	-0.701702632419938\\
2.5	-0.703010168490371\\
3	-0.699696630405979\\
3.5	-0.703065582508843\\
4	-0.699873929369634\\
};
\addlegendentry{TTL ideal sim}

\end{axis}
\end{tikzpicture}%

==> Figs/Utility_log_comparison_all.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
%
\begin{tikzpicture}

\begin{axis}[%
axis line style = thick,
width=2.8in,
height=2.2in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=4,
xlabel style={font=\color{white!15!black}},
xlabel={Delay ratio to inter-request time},
ymin=-1.7,
ymax=-1.1,
ylabel style={font=\color{white!15!black}},
ylabel={Objective function},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0,0)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);

\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
1e-06	-1.12966240488476\\
0.5	-1.12966240476301\\
1	-1.12966240476844\\
1.5	-1.12966240479086\\
2	-1.12966240465747\\
2.5	-1.12966240464946\\
3	-1.12966240465039\\
3.5	-1.12966240493604\\
4	-1.12966240463698\\
};
\addlegendentry{TTL opt ideal}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
1e-06	-1.13697136172741\\
0.5	-1.15122899326388\\
1	-1.15690273328165\\
1.5	-1.16623298221855\\
2	-1.16625978889864\\
2.5	-1.17252953944364\\
3	-1.1754493685523\\
3.5	-1.17354273132635\\
4	-1.18498124042743\\
};
\addlegendentry{LRU}

\addplot [color=mycolor3, mark=o, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
1e-06	-1.3278146718167\\
0.5	-1.3334479332577\\
1	-1.34941408456086\\
1.5	-1.35633016661075\\
2	-1.36391889020551\\
2.5	-1.36640065738798\\
3	-1.38705556077157\\
3.5	-1.38170612844362\\
4	-1.38138210393937\\
};
\addlegendentry{TTL LRU opt sim}

\addplot [color=mycolor4, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
1e-06	-1.32682884176822\\
0.5	-1.34209344903287\\
1	-1.35225777972517\\
1.5	-1.36703018036423\\
2	-1.37478684081461\\
2.5	-1.37886822292388\\
3	-1.38110393273937\\
3.5	-1.37651147512623\\
4	-1.38412449648578\\
};
\addlegendentry{TTL minTTL opt sim}

\addplot [color=mycolor5, mark=asterisk, mark options={solid, mycolor5}]
  table[row sep=crcr]{%
1e-06	-1.12966240488476\\
0.5	-1.20790265379337\\
1	-1.27959426373303\\
1.5	-1.34583640404561\\
2	-1.40746098663175\\
2.5	-1.46511486351107\\
3	-1.51931227916886\\
3.5	-1.57046968838442\\
4	-1.61892967554906\\
};
\addlegendentry{TTL opt ideal 0}
\addplot [color=black, only marks, mark=square, mark options={solid, black}]
  table[row sep=crcr]{%
1e-06	-1.12844410554183\\
0.5	-1.12534633958246\\
1	-1.12768314190262\\
1.5	-1.12828081839007\\
2	-1.13000049331269\\
2.5	-1.1255184780456\\
3	-1.12536707394913\\
3.5	-1.1303414024542\\
4	-1.12929849755517\\
};
\addlegendentry{new pol}
\end{axis}
\end{tikzpicture}%
